Transience in Countable MDPs

The Transience objective is not to visit any state infinitely often. While this is not possible in finite Markov Decision Process (MDP), it can be satisfied in countably infinite ones, e.g., if the transition graph is acyclic. We prove the following fundamental properties of Transience in countably infinite MDPs. 1. There exist uniformly $\epsilon$-optimal MD strategies (memoryless deterministic) for Transience, even in infinitely branching MDPs. 2. Optimal strategies for Transience need not exist, even if the MDP is finitely branching. However, if an optimal strategy exists then there is also an optimal MD strategy. 3. If an MDP is universally transient (i.e., almost surely transient under all strategies) then many other objectives have a lower strategy complexity than in general MDPs. E.g., $\epsilon$-optimal strategies for Safety and co-B\"uchi and optimal strategies for $\{0,1,2\}$-Parity (where they exist) can be chosen MD, even if the MDP is infinitely branching.

==> eps01.tex <==


\begin{theorem}\label{thm:coBuchi}
If an MDP admits uniform $\epsilon$-optimal
MD strategies for all safety objectives, then it also
admits uniform $\epsilon$-optimal
MD strategies for all co-B\"uchi objectives.
\end{theorem}
\begin{proof}
Let $\mdp=\mdptuple$ be an MDP that admits uniform $\epsilon$-optimal
MD strategies for all safety objectives, 
$\coloring:\states\to \{0,1\}$, and $\formula=\Parity{\coloring}$ be the
co-B\"uchi objective.

We show that there exist uniform $\epsilon$-optimal
MD strategies for $\formula$.
I.e., for every $\epsilon >0$ there is an MD strategy $\zstrat_\epsilon$ 
with $\forall_{\state_0 \in \states}\probm_{\mdp,\state_0,\zstrat_\epsilon}(\formula) \ge
\valueof{\mdp}{\state_0} - \epsilon$.

To construct this MD strategy strategy $\zstrat_\epsilon$, we first need several
auxiliary notions.

Let $\epsilon_1 >0$ be a suitably small number (to be determined later)
and $\tau_1 \eqdef 1-\epsilon_1 >0$.
Let $\tau_2 \eqdef 1 - \epsilon_1/k + \lambda$ for a suitably large $k \ge 1$ (to be
determined later) and let $\lambda < \epsilon_1/k$ (e.g., $\lambda \eqdef \epsilon_1/(2k)$). 
Thus $\tau_2 <1$.

Let $\reachset \eqdef \coloring^{-1}(\{1\})$ be the set of states with color $1$
and $\safety{\reachset}$ the safety objective.
We have that $\formula = \eventually \always (\states\setminus\reachset)$.

By our assumption on $\mdp$, there exists a uniformly $\lambda$-optimal
MD strategy $\optav$ for $\safety{\reachset}$.
Let $\states' \eqdef \safesub{\mdp,\optav,\safety{\reachset}}{\tau_1}$
as by Def.~\ref{def:safeset}.
In particular $\states' \subseteq \states\setminus\reachset$, since $\tau_1 >0$.
From $\mdp$ we obtain a modified MDP $\mdp'$ by fixing all player choices from states in
$\states'$ according to $\optav$.

We show that the value w.r.t.\ objective $\formula$
is only slightly smaller in $\mdp'$, i.e.,
\begin{equation}\label{thm:coBuchi:small-loss}
\valueof{\mdp'}{\state_0} \ge \valueof{\mdp}{\state_0} - \epsilon_1
\quad\mbox{for every $\state_0 \in \states$.}
\end{equation}
Let $\state_0 \in \states$.
By definition of the value $\valueof{\mdp}{\state_0}$, 
for every $\delta>0$ there exists a strategy $\zstrat_\delta$ in $\mdp$ from $\state_0$
s.t.\ $\probm_{\mdp,\state_0,\zstrat_\delta}(\formula) \ge \valueof{\mdp}{\state_0} -\delta$.
We define a strategy $\zstrat_\delta'$ in $\mdp'$ from state $\state_0$ as
follows.
First play like $\zstrat_\delta$. If and when a state in $\states'$ is
reached, then henceforth play like $\optav$. This is possible, since no moves
from states outside $\states'$ have been fixed in $\mdp'$,
and all moves from states inside $\states'$ have been fixed 
according to $\optav$.
Then we have:
\[
\begin{aligned}
&\probm_{\mdp',\state_0,\zstrat_\delta'}(\formula) \\[1mm]
&=   \probm_{\mdp,\state_0,\zstrat_\delta}(\formula) \\
& 
\quad \;  - \, \probm_{\mdp,\state_0,\zstrat_\delta}(\eventually \states') \cdot 
\probm_{\mdp,\state_0,\zstrat_\delta}(\formula \mid \eventually \states') \\                                           
&  \quad \; + \,\probm_{\mdp,\state_0,\zstrat_\delta}(\eventually \states') \cdot
\probm_{\mdp',\state_0,\zstrat_\delta'}(\formula \mid \eventually \states') \\[1mm]
& \ge   \probm_{\mdp,\state_0,\zstrat_\delta}(\formula) \\
&      
\quad \;- \,  \probm_{\mdp,\state_0,\zstrat_\delta}(\eventually \states') \cdot 
\probm_{\mdp,\state_0,\zstrat_\delta}(\formula \mid \eventually \states')  \\                                         
& \quad \; + \, \probm_{\mdp,\state_0,\zstrat_\delta}(\eventually \states') \cdot \tau_1 \\[1mm]
& \ge  \valueof{\mdp}{\state_0} - \delta - \probm_{\mdp,\state_0,\zstrat_\delta}(\eventually
\states')(1-\tau_1)\\[1mm]
& \ge  \valueof{\mdp}{\state_0} - \delta - \epsilon_1
\end{aligned}
\]
Since this holds for every $\delta >0$ we have
$\valueof{\mdp'}{\state_0} \ge \valueof{\mdp}{\state_0} - \epsilon_1$, thus (\ref{thm:coBuchi:small-loss}).

Let $\states'' \eqdef \safesub{\mdp,\optav,\safety{\reachset}}{\tau_2-\lambda}$
as by Def.~\ref{def:safeset}.
In particular, $\states'' = \safesub{\mdp',\optav,\safety{\reachset}}{\tau_2-\lambda}$,
since $\optav$ is a uniform MD strategy that has been fixed on the subset $\states'$
in the step from $\mdp$ to $\mdp'$.

Let $\state_0\in \states$ be an arbitrary state.
By definition of the value w.r.t.\ $\formula$ of $\state_0$, for every $\epsilon' >0$ there exists a 
strategy $\zstrat_{\epsilon'}$ from $\state_0$ in $\mdp'$ with
$\probm_{\mdp',\state_0,\zstrat_{\epsilon'}}(\formula) \ge
\valueof{\mdp'}{\state_0} -\epsilon'$.

Since $\tau_2 <1$, can we apply Lemma~\ref{lem:as012-return-to-safe} and obtain
$\probm_{\mdp',\state_0,\hat{\zstrat}}(\eventually \safesub{\mdp',\safety{\reachset}}{\tau_2}) \ge
\probm_{\mdp',\state_0,\hat{\zstrat}}(\formula)$ for every strategy
$\hat{\zstrat}$ from $\state_0$ and
thus in particular for $\zstrat_{\epsilon'}$.

Therefore, $\probm_{\mdp',\state_0,\zstrat_{\epsilon'}}(\eventually \safesub{\mdp',\safety{\reachset}}{\tau_2}) \ge
\valueof{\mdp'}{\state_0} -\epsilon'$.
Since this holds for every $\epsilon' >0$,
in $\mdp'$ the value of $\state_0$ w.r.t.\ the reachability objective 
$\eventually \safesub{\mdp',\safety{\reachset}}{\tau_2}$ is
$\ge \valueof{\mdp'}{\state_0}$ for every state $\state_0$. 

By Theorem~\ref{thm:reach-eps}, for every $\epsilon_2 >0$
there exists a uniformly $\epsilon_2$-optimal MD strategy $\zstrat'$
in $\mdp'$ for this reachability objective.
So we obtain
\begin{equation}\label{thm:coBuchi:reachcore}
\probm_{\mdp',\state_0,\zstrat'}(\eventually \safesub{\mdp',\safety{\reachset}}{\tau_2}) \ge
\valueof{\mdp'}{\state_0} - \epsilon_2\quad\mbox{for every state $\state_0$}.
\end{equation}

In particular, $\zstrat'$ must coincide with $\optav$
at all states in $\states'$, since in $\mdp'$ these choices are
already fixed.

Since $\sigma$ is a uniform $\lambda$-optimal MD strategy for
$\safety{\reachset}$ in $\mdp$ and $\mdp'$,
we have
$
\safesub{\mdp',\safety{\reachset}}{\tau_2} \subseteq
\safesub{\mdp',\sigma,\safety{\reachset}}{\tau_2-\lambda} = \states''
$
and thus by (\ref{thm:coBuchi:reachcore}) we get
\begin{equation}\label{thm:coBuchi:reachcore2}
\probm_{\mdp',\state_0,\zstrat'}(\eventually \states'') \ge
\probm_{\mdp',\state_0,\zstrat'}(\eventually
\safesub{\mdp',\safety{\reachset}}{\tau_2}) \ge
\valueof{\mdp'}{\state_0} - \epsilon_2.
\end{equation}

We obtain the MD strategy $\zstrat_\epsilon$ in $\mdp$ by 
combining the MD strategies $\zstrat'$ and $\optav$.
The strategy $\zstrat_\epsilon$ plays like
$\optav$ at all states inside $\states'$ and like
$\zstrat'$ at all states outside $\states'$ (i.e., at $\states \setminus \states'$).

In order to show that $\zstrat_\epsilon$ has the required property
$\probm_{\mdp,\state_0,\zstrat_\epsilon}(\formula) \ge \valueof{\mdp}{\state_0} - \epsilon$, we 
first estimate the probability that a play according to $\zstrat_\epsilon$ will never
leave the set $\states'$ after having visited a state in
$\states''$.

Let $\state \in \states''$. 
Then, by Lemma~\ref{lem:safe-two-levels},
\begin{equation}\label{thm:coBuchi:stayonion}
\begin{aligned}
\probm_{\mdp,\state,\optav}(\always \states') &\quad\ge \quad \frac{(\tau_2 -\lambda) - \tau_1}{1 - \tau_1}\\[1mm] 
	& \quad= \quad \frac{(1-\epsilon_1/k) - (1-\epsilon_1)}{\epsilon_1}\\ 
	& \quad= \quad  1-\frac{1}{k}\,.
\end{aligned}
\end{equation} 
In particular we also have 
$\probm_{\mdp,\state,\zstrat_\epsilon}(\always \states') \ge 
1-\frac{1}{k}$,
since $\zstrat_\epsilon$ coincides with $\optav$ inside the set
$\states'$.
Finally we obtain for every $\state_0 \in \states$
\[
\begin{array}{lcll}
\probm_{\mdp,\state_0,\zstrat_\epsilon}(\formula)
& = & \probm_{\mdp,\state_0,\zstrat_\epsilon}(\eventually \always
(\states\setminus\reachset)) & \mbox{by def. of $\formula$}\\
& \ge & 
\probm_{\mdp,\state_0,\zstrat_\epsilon}(\eventually \states'')\\
&\quad&
{}\cdot
\probm_{\mdp,\state_0,\zstrat_\epsilon}(\eventually\always \states' \mid
\eventually \states'') & \mbox{since $\states' \subseteq \states\setminus\reachset$}\\[1mm]
& \ge &
\probm_{\mdp',\state_0,\zstrat'}(\eventually \states'') 
\cdot (1-1/k) & \mbox{by (\ref{thm:coBuchi:stayonion})}
\\[1mm]
& \ge &
(\valueof{\mdp'}{\state_0} - \epsilon_2)
\cdot
(1-1/k) & \mbox{by (\ref{thm:coBuchi:reachcore2})} \\[1mm]
& \ge & (\valueof{\mdp}{\state_0} - \epsilon_1 - \epsilon_2)
\cdot (1-1/k) & \mbox{by (\ref{thm:coBuchi:small-loss})}
\end{array}
\]
This holds for every $1 > \epsilon_1, \epsilon_2 >0$ and 
every $k \ge 1$, and moreover $\valueof{\mdp}{\state_0} \le 1$.
Thus we can set $\epsilon_1 = \epsilon_2 \eqdef \epsilon/4$ and 
$k \eqdef \frac{2}{\epsilon}$ 
and obtain $\probm_{\mdp,\state_0,\zstrat_\epsilon}(\formula) 
\ge \valueof{\mdp}{\state_0} -\epsilon$ for every $\state_0 \in \states$ as required.
\end{proof}


The precondition of \cref{thm:coBuchi} (uniform $\epsilon$-optimal
MD strategies for safety objectives) is satisfied by many classes of MDPs,
e.g., the following.

\begin{corollary}\label{cor:coBuchi}
\
\begin{enumerate}
\item
Finitely branching MDPs and acyclic \todo{resp. transient} MDPs admit uniform $\epsilon$-optimal
MD strategies for co-B\"uchi objectives.
\item
Every MDP admits $\epsilon$-optimal deterministic Markov-strategies for co-B\"uchi
objectives.
\end{enumerate}
\end{corollary}
\begin{proof}
Towards (1), finitely branching MDPs trivially admit even uniform optimal MD strategies for safety. 
For acyclic \todo{resp. transient} MDPs this follows from
\Cref{thm:eps-optimal-safety} \todo{resp. \cref{thm:eps-optimal-safety}}.
Then apply \cref{thm:coBuchi}.

Towards (2), every MDP $\mdp$ with a given initial state $\state_0$
  can be transformed into an acyclic MDP $\mdp'$ by encoding a step-counter.
  Then apply (1) to $\mdp'$ to obtain an $\epsilon$-optimal
  MD strategy $\zstrat'$ for co-B\"uchi from its initial state $(\state_0,0)$.
  Finally transform $\zstrat'$ into an $\epsilon$-optimal Markov-strategy
  $\zstrat$ from $\state_0$ in the original MDP $\mdp$.
\end{proof}

